New geometric receipts for design of photonic crystals and metamaterials: optimal toric packings

Design of photonic crystals having large bandgaps above a prescribed band is a well-known physical problem with many applications. A connection to an interesting mathematical construction was pointed out some time ago: it had been conjectured that optimal structures for gaps between bands n and n+1 correspond, in case of transverse magnetic polarisation, to rods located at the generators of centroidal Voronoi tessellation (CVT), and in case of transverse electric polarisation to the walls of this tessellation. We discover another mathematical receipt which produces even better solutions: optimal packing of discs in square and triangular tori. It provides solutions qualitatively different from CVT, sometimes increasing the resulting bandgap size in several times. We therefore introduce two new classes of periodic structures with remarkable properties which may find applications in many other areas of modern solid state physics: arrays of particles located at the centers of optimally packed discs on tori, and nets corresponding to the walls of their Voronoi tessellations.

==> preamble.tex <==
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{physics}
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage[left=23mm,right=13mm,top=35mm,columnsep=15pt]{geometry} 
\usepackage{adjustbox}
\usepackage{placeins}
\usepackage[T1]{fontenc}
\usepackage{lipsum}
\usepackage{csquotes}


